Updating CLIP to Prefer Descriptions Over Captions

Although CLIPScore is a powerful generic metric that captures the similarity between a text and an image, it fails to distinguish between a caption that is meant to complement the information in an image and a description that is meant to replace an image entirely, e.g., for accessibility. We address this shortcoming by updating the CLIP model with the Concadia dataset to assign higher scores to descriptions than captions using parameter efficient fine-tuning and a loss objective derived from work on causal interpretability. This model correlates with the judgements of blind and low-vision people while preserving transfer capabilities and has interpretable structure that sheds light on the caption--description distinction.

==> ig-flats.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.19\linewidth}
    \resizebox{!}{\textwidth}{
    \includegraphics{emnlp2023-latex/images/concadia-flats.png}
    }
    \end{minipage}
    \begin{minipage}{0.78\textwidth}
    \resizebox{\textwidth}{!}{
      \centering
      \setlength{\tabcolsep}{4pt}
        \begin{tabular}{lccl}
        \toprule
        \textbf{Example} & \textbf{Mediation} & \textbf{Score} & \textbf{Attribution} \\
        \midrule
        \multirow{2}{*}{Description} & \xmark & +2.01 & \colorbox{red!9}{\strut a}\colorbox{green!43}{\strut block}\colorbox{green!70}{\strut of}\colorbox{green!68}{\strut flats}\colorbox{red!61}{\strut behind}\colorbox{red!88}{\strut a}\colorbox{red!15}{\strut set}\colorbox{red!4}{\strut of}\colorbox{green!41}{\strut high}\colorbox{green!100}{\strut security}\colorbox{red!29}{\strut gates} \\
        & \cmark & +4.00 & \colorbox{red!14}{\strut a}\colorbox{green!33}{\strut block}\colorbox{green!90}{\strut of}\colorbox{green!100}{\strut flats}\colorbox{red!13}{\strut behind}\colorbox{red!51}{\strut a}\colorbox{red!6}{\strut set}\colorbox{red!10}{\strut of}\colorbox{green!4}{\strut high}\colorbox{green!67}{\strut security}\colorbox{red!10}{\strut gates} \\
        \midrule
        \multirow{3}{*}{Caption} & \xmark & -11.16 & \colorbox{red!14}{\strut the}\colorbox{red!60}{\strut exclusive}\colorbox{green!60}{\strut block}\colorbox{green!47}{\strut of}\colorbox{red!31}{\strut flats}\colorbox{red!54}{\strut in}\colorbox{green!6}{\strut chelsea}\colorbox{red!35}{\strut ,}\colorbox{red!18}{\strut london}\colorbox{red!60}{\strut that}\colorbox{red!83}{\strut were}\colorbox{red!100}{\strut used}\colorbox{green!0}{\strut as}\colorbox{red!15}{\strut the}\colorbox{red!2}{\strut exterior}\colorbox{red!18}{\strut of}\colorbox{red!50}{\strut mark}\colorbox{green!20}{\strut 's}\colorbox{green!12}{\strut flat} \\
        & \cmark & -11.43 & \colorbox{red!3}{\strut the}\colorbox{red!100}{\strut exclusive}\colorbox{red!32}{\strut block}\colorbox{green!54}{\strut of}\colorbox{red!18}{\strut flats}\colorbox{red!91}{\strut in}\colorbox{green!50}{\strut chelsea}\colorbox{red!46}{\strut ,}\colorbox{red!12}{\strut london}\colorbox{red!67}{\strut that}\colorbox{red!63}{\strut were}\colorbox{red!59}{\strut used}\colorbox{red!22}{\strut as}\colorbox{red!17}{\strut the}\colorbox{red!26}{\strut exterior}\colorbox{red!12}{\strut of}\colorbox{red!72}{\strut mark}\colorbox{red!7}{\strut 's}\colorbox{green!24}{\strut flat} \\
        \bottomrule
        \end{tabular}
    }
    \end{minipage}
    \caption{Integrated gradient attributions for a sample image and its corresponding description and caption from the Concadia dataset.}
    \label{fig:ig-attribution}
\end{figure*}

==> ig-horse.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.19\linewidth}
    \resizebox{!}{\textwidth}{
    \includegraphics{emnlp2023-latex/images/concadia-horse.png}
    }
    \end{minipage}
    \begin{minipage}{0.78\textwidth}
    \resizebox{\textwidth}{!}{
      \centering
      \setlength{\tabcolsep}{4pt}
        \begin{tabular}{lccl}
        \toprule
        \textbf{Example} & \textbf{Mediation} & \textbf{Score} & \textbf{Attribution} \\
        \midrule
        \multirow{2}{*}{Description} & \xmark & +13.6 & \colorbox{red!0}{\strut a}\colorbox{red!6}{\strut bay}\colorbox{green!100}{\strut horse}\colorbox{green!13}{\strut can}\colorbox{green!11}{\strut tering}\colorbox{green!42}{\strut across}\colorbox{red!11}{\strut a}\colorbox{green!16}{\strut grassy}\colorbox{green!6}{\strut field}\colorbox{green!7}{\strut with}\colorbox{red!14}{\strut a}\colorbox{green!8}{\strut fence}\colorbox{green!0}{\strut in}\colorbox{green!2}{\strut the}\colorbox{green!17}{\strut background}\colorbox{red!7}{\strut .} \\
        & \cmark & +8.66 & \colorbox{green!11}{\strut a}\colorbox{red!8}{\strut bay}\colorbox{green!100}{\strut horse}\colorbox{green!14}{\strut can}\colorbox{red!10}{\strut tering}\colorbox{green!51}{\strut across}\colorbox{red!7}{\strut a}\colorbox{green!46}{\strut grassy}\colorbox{green!5}{\strut field}\colorbox{green!9}{\strut with}\colorbox{red!12}{\strut a}\colorbox{green!16}{\strut fence}\colorbox{red!2}{\strut in}\colorbox{green!6}{\strut the}\colorbox{green!22}{\strut background}\colorbox{red!9}{\strut .} \\
        \midrule
        \multirow{3}{*}{Caption} & \xmark & -13.4 & \colorbox{red!10}{\strut a}\colorbox{green!48}{\strut cleveland}\colorbox{red!3}{\strut bay}\colorbox{red!69}{\strut /}\colorbox{red!52}{\strut hol}\colorbox{red!100}{\strut steiner}\colorbox{green!0}{\strut cross} \\
        & \cmark & -5.22 & \colorbox{red!5}{\strut a}\colorbox{green!59}{\strut cleveland}\colorbox{red!2}{\strut bay}\colorbox{red!60}{\strut /}\colorbox{red!19}{\strut hol}\colorbox{red!100}{\strut steiner}\colorbox{green!24}{\strut cross} \\
        \bottomrule
        \end{tabular}
    }
    \end{minipage}
    \caption{Integrated gradient attributions for a sample image and its corresponding description and caption from the Concadia dataset.}
    \label{fig:ig-attribution}
\end{figure*}

==> ig-sting.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.19\linewidth}
    \resizebox{!}{\textwidth}{
    \includegraphics{emnlp2023-latex/images/concadia-sting.png}
    }
    \end{minipage}
    \begin{minipage}{0.78\textwidth}
    \resizebox{\textwidth}{!}{
      \centering
      \setlength{\tabcolsep}{4pt}
        \begin{tabular}{lccl}
        \toprule
        \textbf{Example} & \textbf{Mediation} & \textbf{Score} & \textbf{Attribution} \\
        \midrule
        \multirow{2}{*}{Description} & \xmark & +12.9 & \colorbox{green!23}{\strut sting}\colorbox{green!56}{\strut wearing}\colorbox{red!7}{\strut a}\colorbox{green!33}{\strut red}\colorbox{green!12}{\strut long}\colorbox{red!1}{\strut coat}\colorbox{green!42}{\strut standing}\colorbox{red!15}{\strut in}\colorbox{red!8}{\strut a}\colorbox{green!100}{\strut wrestling}\colorbox{green!11}{\strut ring}\colorbox{red!4}{\strut talking}\colorbox{red!4}{\strut on}\colorbox{red!11}{\strut a}\colorbox{green!18}{\strut microphone} \\
        & \cmark & +5.94 & \colorbox{green!0}{\strut sting}\colorbox{green!8}{\strut wearing}\colorbox{red!13}{\strut a}\colorbox{green!46}{\strut red}\colorbox{green!23}{\strut long}\colorbox{green!27}{\strut coat}\colorbox{green!100}{\strut standing}\colorbox{green!7}{\strut in}\colorbox{green!0}{\strut a}\colorbox{green!53}{\strut wrestling}\colorbox{green!8}{\strut ring}\colorbox{green!6}{\strut talking}\colorbox{green!7}{\strut on}\colorbox{red!6}{\strut a}\colorbox{green!35}{\strut microphone} \\
        \midrule
        \multirow{3}{*}{Caption} & \xmark & -14.3 & \colorbox{red!100}{\strut sting}\colorbox{red!27}{\strut (}\colorbox{green!28}{\strut pictured}\colorbox{red!17}{\strut in}\colorbox{red!42}{\strut 2}\colorbox{red!42}{\strut 0}\colorbox{red!31}{\strut 1}\colorbox{red!12}{\strut 5}\colorbox{red!11}{\strut )}\colorbox{green!6}{\strut went}\colorbox{red!66}{\strut on}\colorbox{red!4}{\strut to}\colorbox{red!19}{\strut win}\colorbox{green!1}{\strut the}\colorbox{green!80}{\strut tna}\colorbox{green!21}{\strut world}\colorbox{green!18}{\strut heavyweight}\colorbox{red!25}{\strut championship}\colorbox{green!2}{\strut at}\colorbox{red!36}{\strut bound}\colorbox{green!4}{\strut for}\colorbox{red!53}{\strut glory}\colorbox{red!33}{\strut iv}\colorbox{red!11}{\strut .} \\
        & \cmark & -17.7 & \colorbox{red!100}{\strut sting}\colorbox{red!43}{\strut (}\colorbox{red!12}{\strut pictured}\colorbox{red!24}{\strut in}\colorbox{red!51}{\strut 2}\colorbox{red!64}{\strut 0}\colorbox{red!50}{\strut 1}\colorbox{red!27}{\strut 5}\colorbox{red!14}{\strut )}\colorbox{red!31}{\strut went}\colorbox{red!71}{\strut on}\colorbox{green!7}{\strut to}\colorbox{red!34}{\strut win}\colorbox{red!9}{\strut the}\colorbox{green!12}{\strut tna}\colorbox{green!1}{\strut world}\colorbox{red!18}{\strut heavyweight}\colorbox{red!22}{\strut championship}\colorbox{green!6}{\strut at}\colorbox{red!15}{\strut bound}\colorbox{green!8}{\strut for}\colorbox{red!48}{\strut glory}\colorbox{red!33}{\strut iv}\colorbox{green!8}{\strut .} \\
        \bottomrule
        \end{tabular}
    }
    \end{minipage}
    \caption{Integrated gradient attributions for a sample image and its corresponding description and caption from the Concadia dataset.}
    \label{fig:ig-attribution}
\end{figure*}

==> ig-warrior.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{0.19\linewidth}
    \resizebox{!}{\textwidth}{
    \includegraphics{emnlp2023-latex/images/concadia-warrior.png}
    }
    \end{minipage}
    \begin{minipage}{0.78\textwidth}
    \resizebox{\textwidth}{!}{
      \centering
      \setlength{\tabcolsep}{4pt}
        \begin{tabular}{lccl}
        \toprule
        \textbf{Example} & \textbf{Mediation} & \textbf{Score} & \textbf{Attribution} \\
        \midrule
        \multirow{2}{*}{Description} & \xmark & +10.9 & \colorbox{green!4}{\strut a}\colorbox{green!100}{\strut portrait}\colorbox{green!33}{\strut of}\colorbox{red!3}{\strut a}\colorbox{green!11}{\strut male}\colorbox{green!11}{\strut with}\colorbox{red!15}{\strut a}\colorbox{red!0}{\strut long}\colorbox{green!13}{\strut beard}\colorbox{green!15}{\strut wearing}\colorbox{red!0}{\strut a}\colorbox{green!29}{\strut hat}\colorbox{red!3}{\strut and}\colorbox{red!3}{\strut a}\colorbox{red!13}{\strut fur}\colorbox{red!0}{\strut -}\colorbox{red!1}{\strut colla}\colorbox{green!10}{\strut red}\colorbox{red!0}{\strut coat} \\
        & \cmark & +7.22 & \colorbox{red!2}{\strut a}\colorbox{green!100}{\strut portrait}\colorbox{green!18}{\strut of}\colorbox{red!5}{\strut a}\colorbox{green!31}{\strut male}\colorbox{green!2}{\strut with}\colorbox{red!15}{\strut a}\colorbox{green!30}{\strut long}\colorbox{green!24}{\strut beard}\colorbox{green!11}{\strut wearing}\colorbox{red!5}{\strut a}\colorbox{green!17}{\strut hat}\colorbox{red!6}{\strut and}\colorbox{red!3}{\strut a}\colorbox{red!7}{\strut fur}\colorbox{red!0}{\strut -}\colorbox{green!2}{\strut colla}\colorbox{green!11}{\strut red}\colorbox{green!9}{\strut coat} \\
        \midrule
        \multirow{3}{*}{Caption} & \xmark & -7.13 & \colorbox{red!22}{\strut the}\colorbox{red!100}{\strut division}\colorbox{red!25}{\strut was}\colorbox{red!2}{\strut named}\colorbox{red!3}{\strut after}\colorbox{red!4}{\strut the}\colorbox{green!19}{\strut medieval}\colorbox{green!19}{\strut albanian}\colorbox{green!9}{\strut warrior}\colorbox{red!7}{\strut sk}\colorbox{green!6}{\strut ander}\colorbox{green!22}{\strut beg}\colorbox{red!11}{\strut .} \\
        & \cmark & -9.65 &  \colorbox{red!25}{\strut the}\colorbox{red!100}{\strut division}\colorbox{red!42}{\strut was}\colorbox{red!61}{\strut named}\colorbox{red!21}{\strut after}\colorbox{red!11}{\strut the}\colorbox{green!24}{\strut medieval}\colorbox{green!8}{\strut albanian}\colorbox{green!14}{\strut warrior}\colorbox{red!8}{\strut sk}\colorbox{green!3}{\strut ander}\colorbox{green!31}{\strut beg}\colorbox{red!23}{\strut .} \\
        \bottomrule
        \end{tabular}
    }
    \end{minipage}
    \caption{Integrated gradient attributions for a sample image and its corresponding description and caption from the Concadia dataset.}
    \label{fig:ig-attribution}
\end{figure*}
